A Survey of Transformer Enabled Time Series Synthesis

Generative AI has received much attention in the image and language domains, with the transformer neural network continuing to dominate the state of the art. Application of these models to time series generation is less explored, however, and is of great utility to machine learning, privacy preservation, and explainability research. The present survey identifies this gap at the intersection of the transformer, generative AI, and time series data, and reviews works in this sparsely populated subdomain. The reviewed works show great variety in approach, and have not yet converged on a conclusive answer to the problems the domain poses. GANs, diffusion models, state space models, and autoencoders were all encountered alongside or surrounding the transformers which originally motivated the survey. While too open a domain to offer conclusive insights, the works surveyed are quite suggestive, and several recommendations for best practice, and suggestions of valuable future work, are provided.

==> component_paragraphs/Prior_art/Standard-scope.tex <==
\subsection{Scope}\label{sect::scope}
The scope of this survey is set by a definition of the narrow intersection of time series generation and TNN enabled models. This section provides these definitions, after which section \ref{sect::reviewed_works} reviews selected works.
\input{component_paragraphs/Prior_art/what_is_time_series_generation}
\input{component_paragraphs/Prior_art/what_is_transformer_enabled}

==> component_paragraphs/to_be_deployed/Suggestions_for_future_work_based_on_the_survey.tex <==
\hl{Surveys often include a suggestions section where the lessons learned during the survey suggest future research directions}

==> component_paragraphs/to_be_deployed/Value_of_TSG.tex <==
Time series generation is cited as having four primary motivations. Data augmentation to correct imbalanced datasets

==> component_paragraphs/to_be_deployed/arguments.tex <==
Survey coverage:

Many surveys of generative methods do not provide good coverage of the time series domain methods \cite{GAN_survey, GAI_survey, Medical_cGANs, Synthetic_data_gen_survey} \hl{add more}. Surveys targeting the domain, in turn, rarely explore TNN based methods, at best covering one or two implementations \cite{GAN_in_TS_survey, TSG_benchmark, time_series_data_aug_survey, No_TGANS_and_results_of_fiddling, TSGAN_comparison}. This gap in coverage might be explained by a compounding of scarcities. The challenges of GAN research, the lower degree of attention to time series domain GANs, and the novelty of the TNN relative to temporal convolutional network (TCN) and RNN implementations in this domain may plausibly have limited the number of implementations to report. This work reports on \hl{number of implementations} that meet its standard for inclusion, and thereby fill this gap in the literature.

%--------------------------------------------------------------------------------------------------------------
Lack of comparison:

Time series generation models are rarely evaluated on comparable tasks \cite{TSG_benchmark, TSGAN_comparison}.



%how much better performance is being purchased for how much more training/paramater count and inference time? If LLM models mostly do dynamic decoding, should comparisons only be done on a time horizon of 1.

%--------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------

==> component_paragraphs/to_be_deployed/catagorization.tex <==
Forecasting/synthesis
supervised/unsupervised
univariate/multivariate
GAN/not gan - for synthisizers
horison type - for forecasters
domain of application (stock market, bio signals, general, geological, etc...)


Big table values:
    title, type(forecasting, GAN, diffusion, AE), year published, publication venue, github link if available

Taxonomize

Hypothetical sections:

LLM based vs not

Do include datasets used.

Maybe, since the focus is on a smaller number of works, focus on the means of evaluation and particular methods, expanding rather than contracting? Also refer readers to the surveys whenever possible to avoid redundancy.

Salient divide between models that treat a TD segment as one input or as D inputs. At least one does BOTH.
Code availability,
Data availability
Used evaluation metrics?
Include a reason why each non-synthesis model was included
An evaluation metrics table might be valueable too.

Compared against other models (list models), compared using which metrics (list metrics).

ATS hasn't been compared to any fellows (ARIMA and DeepAR)
Informer hasn't been (ARIMA)
TTS-CGAN hasn't. (TimeGAN)
TTS-GAN hasn't (TimeGAN)
TimeWeaver hasn't, and invents its own eval metric.
TsT-GAN (TimeGAN)
MTS-CGAN None.
Time-Transformer AAE (TimeGAN)
DSAT-ECG None
Time-LLM: Informer
TimesFM: Informer
GenF: Informer

Invents metrics:
    TTS-GAN
    TimeWeaver
    MTS-CGAN


Informer - Pure TNN, forecaster, countermeasure to autoencoder error.
AST - GAN, hybrid (aux) architecture (though mostly pure), forecaster, countermeasure to autoencoder error, conditioning.
	ACT - GAN, hybrid (aux)  + hybrid "convolutional attention block", architecture (though mostly pure), forecaster, countermeasure to autoencoder error, conditioning.
GenF - forecaster, hybrid architecture, countermeasure to autoencoder error.
TTS-GAN - Pure TNN GAN, synthesis, lineage founder*.
TsT-GAN - Pure TNN GAN, synthesis, countermeasure to autoencoder error.
TTS-CGAN - relativley Pure TNN GAN (aux), synthesis, lineage*, conditioning.
MTS-CGAN - relativley Pure TNN GAN (aux), synthesis, lineage*, conditioning.
Time-LLM - relativley Pure TNN, Large model, forecaster
DSAT-ECG - Hybrid model, Diffusion, synthesis, conditioning
Time-Transformer AAE - Autoencoder, synthesis, hybrid (aux) + hybrid Time-Transformer module
TimesFM - relativley Pure TNN, large model, forecasting
Time Weaver - Hybrid diffusion, conditioning, synthesis

Forecasters vs Synthisizers
Pure TNN vs Hybrid
countermeasure to autoencoder error

==> component_paragraphs/to_be_deployed/offerings.tex <==
What do each of the surveys offer the reader of their subject?

\cite{Logan_PM_XAI_survey}, unique among the surveys, was edited by the same PIs as the present work, and should be attended to in all matters of style and content.

    Introduction:
        The intro section commits a zoom in: Technology -> industrial revols. -> the 4th such -> focus on maintenance and uptime -> PdM -> the rising signif. of human understanding and man-machine-teaming -> ind. 5.0 -> the relevance of XAI and iML -> statment of works contribution:
            1. survey using PRISMA of XAI/iML over PdM domain.
            2. Catagorization of XAI/iML methods seen.
            3. List seen challanges.

        Lessons:
            Zoom in from biggest pic to smallest. Justify the target. Mention contributions. Contributions should include a catagorization of found info, such as what, and how sucessfully, is done. Also a list of challanges.

    Background is for defining terms.

Several archs (AST, GenF, Informer, TsT-GAN, TTAAE) are concerend with ballancing next-step modeling and global modeling,
at least AST and TTAAE employ auxiliary discriminators.
Hybrid models seem more sucessful than pure ones, both in training modality (not just forecasters but adversarial forecasters, not just generators but adversarial generators) and modules (non pure archatectures).

At leat two models TTAAE and DSAT-ECG have distinct hybrid archatectures for global and local dependency modeling.


==> component_paragraphs/to_be_deployed/state_of_the_art.tex <==
\hl{The survey credit section might make this redundant, so I suggest they merge}

==> tables_and_figures/tables/works_table.tex <==
\ifbool{dismember}
{
\begin{table}\label{method_tab}
\centering
\begin{tabular}{|c c|}
    \hline
    Model/Method & Date of publication (arXiv counted)\\
    \hline
    Informer \cite{Informer} & Dec 2020\\
    \hline
    ATS \cite{AST} & Dec 2020\\
    \hline
    GenF \cite{TGAN_uses_informer} & Oct 2021\\
    \hline
    TTS-GAN \cite{Close_competitor} & Feb 2022\\
    \hline
    TsT-GAN \cite{TsT-GAN} & May 2022\\
    \hline
    TTS-CGAN \cite{Closest_competitor, sEMG} & Jun 2022\\
    \hline
    MTS-CGAN \cite{Competitor_sucessor} & Oct 2022\\
    \hline
    TIME-LLM \cite{Time_lama} & Oct 2023\\
    \hline
    DSAT-ECG \cite{DSAT-ECG} & Oct 2023\\
    \hline
    Time-Transformer AAE \cite{TNN_TS_AE} & Dec 2023\\
    \hline
    TimesFM \cite{TimesFM} & Jan 2024\\
    \hline
    Time Weaver \cite{TimeWeaver} & Mar 2024\\
    \hline
\end{tabular}
\end{table}
}
{
\begin{table*}[t]\label{method_tab}
\centering
\begin{tabular}{|c c c c|}
    \hline
    Model/Method & Date of publication (arXiv counted) & Venue (at time of writing) & Task\\
    \hline
    Informer \cite{Informer} & Dec 2020 & AAAI Conference on Artificial Intelligence & Forecasting\\
    \hline
    ATS \cite{AST} & Dec 2020 & Neural Information Processing Systems & Forecasting\\
    \hline
    GenF \cite{TGAN_uses_informer} & Oct 2021 & arXiv & Forecasting\\
    \hline
    TTS-GAN \cite{Close_competitor} & Feb 2022 & Conference on Artificial Intelligence in Medicine in Europe & Synthesis\\
    \hline
    TsT-GAN \cite{TsT-GAN} & May 2022 & arXiv & Synthesis\\
    \hline
    TTS-CGAN \cite{Closest_competitor, sEMG} & Jun 2022 & arXiv & Synthesis\\
    \hline
    MTS-CGAN \cite{Competitor_sucessor} & Oct 2022 & arXiv & Synthesis\\
    \hline
    TIME-LLM \cite{Time_lama} & Oct 2023 & arXiv & Forecasting\\
    \hline
    DSAT-ECG \cite{DSAT-ECG} & Oct 2023 & Italian National Conference on Sensors & Synthesis\\
    \hline
    Time-Transformer AAE \cite{TNN_TS_AE} & Dec 2023 & arXiv & Synthesis\\
    \hline
    TimesFM \cite{TimesFM} & Jan 2024 & arXiv & Forecasting\\
    \hline
    Time Weaver \cite{TimeWeaver} & Mar 2024 & arXiv & Synthesis\\
    \hline
\end{tabular}
\end{table*}
}
